Circumventing the resolution-time tradeoff in Ultrasound Localization Microscopy by Velocity Filtering

Ultrasound Localization Microscopy (ULM) offers a cost-effective modality for microvascular imaging by using intravascular contrast agents (microbubbles). However, ULM has a fundamental trade-off between acquisition time and spatial resolution, which makes clinical translation challenging. In this paper, in order to circumvent the trade-off, we introduce a spatiotemporal filtering operation dubbed velocity filtering, which is capable of separating contrast agents into different groups based on their vector velocities thus reducing interference in the localization step, while simultaneously offering blood velocity mapping at super resolution, without tracking individual microbubbles. As side benefit, the velocity filter provides noise suppression before microbubble localization that could enable substantially increased penetration depth in tissue typically by 4cm or more. We provide a theoretical analysis of the performance of velocity filter. Numerical experiments confirm that the proposed velocity filter is able to separate the microbubbles with respect to the speed and direction of their motion. In combination with subsequent localization of microbubble centers, e.g. by matched filtering, the velocity filter improves the quality of the reconstructed vasculature significantly and provides blood flow information. Overall, the proposed imaging pipeline in this paper enables the use of higher concentrations of microbubbles while preserving spatial resolution, thus helping circumvent the trade-off between acquisition time and spatial resolution. Conveniently, because the velocity filtering operation can be implemented by fast Fourier transforms(FFTs) it admits fast, and potentially real-time realization. We believe that the proposed velocity filtering method has the potential to pave the way to clinical translation of ULM.

==> related.tex <==
\section{Related Work}
\label{chapter2}
A paradigm shift happens in the work by Huang et al. \cite{huang2020short}. They introduced an additional signal processing step, which is a filtering operation, to separate spatially overlapping microbubble signals into sub-populations in order to break the fundamental trade-off between acquisition time and spatial resolution. Microbubbles will be separated based on their spatiotemporal differences in the flow dynamics, i.e. with respect to their velocities and speed. Subsequently, localization and tracking will be performed for each sub-population separately. That leads to more robust ULM imaging of high-concentration microbubble injections. The imaging pipeline suggested by \cite{huang2020short} can be seen in Figure \ref{imagingpipelinehuang}.      
\begin{figure}[hbt!]
\begingroup
    \centering
    \begin{tabular}{c}
\hspace{0cm}{ \includegraphics[width=1\linewidth]{figures/filtersong.PNG}}
\end{tabular}
\caption{Imaging pipeline suggested by \cite{huang2020short}. The figure is from \cite{huang2020short}.}
\label{imagingpipelinehuang}
\endgroup
\end{figure}

The main intuition is that filtering operation increases the possibility of observing isolated microbubbles for high-concentration injections. Subsequently, it eliminates the need of using diluted microbubble injections, that results in shorter acquisition time. Huang et al. \cite{huang2020short} introduced the filtering operation as a prepossessing step for localization and tracking steps. They validate their proposed method by using several experimental setups. First, they validate their method on synthetically generated flow channel phantom which combines real flow phantoms frame-by-frame: a total of four different flow rates and two different directions are used. Additionally, they validate microbubble separation in vivo by using chicken embryo chorioallantoic membrane (CAM) data, chicken CAM tumor and brain data. They state that chicken CAM tumor and chicken brain data are useful to test the method in more complex three-dimensional (3D) vascular networks. Moreover, they investigate the effect of their proposed method on acquisition time which can be seen in Figure \ref{timeacvssat}. This result is obtained for the chicken CAM data. The chicken CAM data has minimal tissue motion and provides a thin vascular bed with complex vessel patterns. The further details for CAM data can be found in \cite{huang2020short}. 

In Figure \ref{timeacvssat}, the vertical axis represents saturation rate for a selected region in vessel structure map. The saturation rate indicates how much the selected vessel lumen is populated by detected microbubble centers. The saturation rate is measured by comparing optical microscopy and ultrasound localization microscopy (ULM). An optical image of the same region of interest is captured and used as ground truth in ULM. In Figure \ref{timeacvssat}, the blue curve is obtained by using the method with microbubble separation while red curve is obtained by using the method without microbubble separation. It can be seen that the acquisition time to achieve a given saturation dropped significantly when microbubble separation was introduced. The selected vessel lumen becomes highly populated within the first 2-3 seconds in the blue curve while the red curve is not able to achieve a similar saturation rate for long acquisition time. The reason for this is that the imaging algorithm becomes capable of identifying smaller size of microvessels quickly when microbubble separation is introduced. Without microbubble separation, localization accuracy is especially low for small size vessels. Inaccurately localized  microbubbles will be removed by the tracking algorithm and hence, identifying or resolving smaller vessels requires long acquisition time. However, introducing microbubble separation increases the localization accuracy and that leads to quickly resolving the microvessel map. So, the method introduced in \cite{huang2020short} could improve the trade-off between spatial resolution and acquisition time in ULM and it might pave the way to clinical translation of ULM.           
\begin{figure}[hbt!]
\begingroup
    \centering
    \begin{tabular}{c}
\hspace{0cm}{ \includegraphics[width=0.7\linewidth]{figures/TAvsSat.PNG}}
\end{tabular}
\caption{Influence of microbubble separation on acquisition time. The figure is from \cite{huang2020short}.}
\label{timeacvssat}
\endgroup
\end{figure}

There are some open problems regarding the filtering operation suggested by Huang et al. \cite{huang2020short}. First, they introduce a cone-shaped filter in spatiotemporal frequency domain. However, the effect of the cone filter on the microbubble signal was not clearly analyzed and fully understood. Subsequently, the cone filter is not fully capable of separating the microbubble signal without any unwanted distortion. Applying sharp cone filters would split the microbubble signal into different passbands that cause the unwanted distortion. In order to minimize that effect, they use large passbands and large overlap between consecutive filters. However, that brings another issue: microbubble doubling. One microbubble signal will be recovered many times by consecutive filters that would lead to overestimate the microbubble density. They state that microbubble doubling would not affect the imaging of vasculature structure or morphology. Another open problem is that even though they state that filtering is based on flow dynamics such as flow speed and directions, there is no solid understanding regarding that. Therefore, tracking is required to detect the microbubble speed and directions. Moreover, another issue is that increasing the number of filtering operation would result in a more robust localization and tracking but it will also significantly increase the computational cost.

The method proposed in this paper builds on the filtering idea suggested by Huang et al. \cite{huang2020short}. Imaging pipeline in \cite{huang2020short} is adopted by removing the tracking step. On the other hand, the proposed method differs from \cite{huang2020short} in the following ways. First, we propose to use a plane-shaped filter in the spatiotemporal frequency domain rather than cone filter. The plane-shaped filter is implemented with a time windowing operator. The reason for time windowing operator will be provided in the following sections. Second, we provide a complete analysis of our proposed filter's effect on microbubble PSFs and provide rigorous mathematical analysis and results. Third, unlike \cite{huang2020short}, our filtering operation would not result in any microbubble signal loss. Additionally, our filter is fully capable of separating the microbubble signals based on both speed and direction. In other words, our filtering approach is sensitive to all speed ranges in all directions and therefore filtering operation provides the microbubble velocity information. Moreover, since the developed filtering operation provides the microbubble velocity information, the tracking step is no longer required. 
